FaceCraft4D: Animated 3D Facial Avatar Generation from a Single Image

We present a novel framework for generating high-quality, animatable 4D avatar from a single image. While recent advances have shown promising results in 4D avatar creation, existing methods either require extensive multiview data or struggle with shape accuracy and identity consistency. To address these limitations, we propose a comprehensive system that leverages shape, image, and video priors to create full-view, animatable avatars. Our approach first obtains initial coarse shape through 3D-GAN inversion. Then, it enhances multiview textures using depth-guided warping signals for cross-view consistency with the help of the image diffusion model. To handle expression animation, we incorporate a video prior with synchronized driving signals across viewpoints. We further introduce a Consistent-Inconsistent training to effectively handle data inconsistencies during 4D reconstruction. Experimental results demonstrate that our method achieves superior quality compared to the prior art, while maintaining consistency across different viewpoints and expressions.

==> images/video_prior.tex <==
\begin{figure*}[t]
  \centering
    \includegraphics[width=1\textwidth]{pdfs/video_prior.pdf}
  \caption{\textbf{Video Prior}: We use the FLAME 3D head model to synthesize multi-view facial expressions, ensuring expression synchronization across views. By combining identity parameters with expression and pose data, and leveraging a video diffusion model, our approach generates expressive, identity-preserving videos from multiple perspectives.}
  \label{fig:video_prior}
\end{figure*}


==> tables/tb_ablation.tex <==
\begin{table}[t]
\centering
\caption{Ablation of reconstruction modules. "Warp" refers to the warping-based control generation (Sec.~\ref{sec:image_prior}) and MA to cross-view mutual attention (Sec.~\ref{sec:image_prior}).}
\label{tb:ablation_reconstruction}
\small
\begin{tabularx}{\linewidth}{l>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X}
\toprule
Method & CLIP-I $\uparrow$ & ID $\uparrow$ & FID \\ 
\midrule
w/o Warp w/o MA & 0.7328 & 0.4787 & 182.27 \\
w/o Warp & 0.7886 & 0.4915 & 171.08 \\
w/o MA & 0.8151 & 0.4951 & 172.43 \\
Full & \textbf{0.8162} & \textbf{0.4984} & \textbf{166.96} \\
\bottomrule
\end{tabularx}
\end{table}

\begin{table}[t]
\centering
\caption{Ablation of animation modules.}
\label{tb:ablation_animation}
\small
\begin{tabularx}{\linewidth}{l>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X}
\toprule
Method & CLIP-I $\uparrow$ & ID $\uparrow$ & FID $\downarrow$ \\ 
\midrule
w/o COIN & 0.7688 & 0.4952 & 144.95 \\
Full & \textbf{0.7729} & \textbf{0.5010} & \textbf{142.80} \\
\bottomrule
\end{tabularx}
\end{table}
